Performance of a Kinetic Inductance Phonon-Mediated Detector at the NEXUS Cryogenic Facility

Microcalorimeters that leverage microwave kinetic inductance detectors to read out phonon signals in the particle-absorbing target, referred to as kinetic inductance phonon-mediated (KIPM) detectors, offer an attractive detector architecture to probe dark matter (DM) down to the fermionic thermal relic mass limit. A prototype KIPM detector featuring a single aluminum resonator patterned onto a 1-gram silicon substrate was operated in the NEXUS low-background facility at Fermilab for characterization and evaluation of this detector architecture's efficacy for a dark matter search. An energy calibration was performed by exposing the bare substrate to a pulsed source of 470 nm photons, resulting in a baseline resolution on the energy absorbed by the phonon sensor of $2.1\pm0.2$ eV, a factor of two better than the current state-of-the-art, enabled by millisecond-scale quasiparticle lifetimes. However, due to the sub-percent phonon collection efficiency, the resolution on energy deposited in the substrate is limited to $\sigma_E=318 \pm 28$ eV. We further model the signal pulse shape as a function of device temperature to extract quasiparticle lifetimes, as well as the observed noise spectra, both of which impact the baseline resolution of the sensor.

==> frontmatter-bak.tex <==
\preprint{APS/123-QED}

\title{Performance of a Kinetic Inductance Phonon-Mediated Detector at the NEXUS Cryogenic Facility}

%% "Tier-1" Authors: order of contribution, PIs last (alphabetical)

\author{Dylan Temples}
    % \altaffiliation[Also at ]{Physics Department, XYZ University.}
    \email{dtemples@fnal.gov}

    \affiliation{Astrophysics Department, Fermi National Accelerator Laboratory (FNAL), Batavia, IL, 60510, USA}

    \affiliation{Emerging Technologies Directorate, Fermi National Accelerator Laboratory (FNAL), Batavia, IL, 60510, USA}


\author{Osmond Wen}
\author{Karthik Ramanathan}
\author{Sunil Golwala}
% %% "Tier-2" Authors: alphabetical
\author{Taylor Aralis}
\author{Yen-Yung Chang}
    \altaffiliation[Presently at ]{Department of Physics, University of California, Berkeley, CA, 94720, USA}

    \affiliation{Division of Physics, Mathematics, and Astronomy, California Institute of Technology, Pasadena, CA, 91106, USA}

\author{Lauren Hsu}
% %% "Tier-2" Authors: alphabetical
\author{Daniel Baxter}
\author{Daniel Bowring}
\author{Samantha Lewis}
    \altaffiliation[Presently at ]{Department of Physics and Astronomy, Wellesley College, Wellesley, MA, 02481, USA}
\author{Patrick Lukens}

    \affiliation{Astrophysics Department, Fermi National Accelerator Laboratory (FNAL), Batavia, IL, 60510, USA}

% %% "Tier-2" Authors: alphabetical
\author{Matthew Hollister}
\author{Christopher James}

    \affiliation{Emerging Technologies Directorate, Fermi National Accelerator Laboratory (FNAL), Batavia, IL, 60510, USA}

\author{Noah Kurinsky}

    \affiliation{Kavli Institute for Particle Astrophysics and Cosmology, SLAC National Accelerator Laboratory, Menlo Park, CA, 94025, USA}
    
% %% "Tier-2" Authors: alphabetical
\author{Ran Chen}
\author{Enectali Figueroa-Feliciano}
\author{Kyle Kennard}
\author{Valentina Novati}
    \altaffiliation[Presently at ]{LPSC, National Centre for Scientific Research, Universit\'{e} Grenoble Alpes, Grenoble, France}
\author{Tom Ren}
\author{Benjamin Schmidt}
    \altaffiliation[Presently at ]{IRFU, Alternative Energies and Atomic Energy Commission, Universit\'{e} Paris-Saclay, France}
    %\altaffiliation[Presently at ]{Institute of Research into the Fundamental Laws of the Universe, Alternative Energies and Atomic Energy Commission, Universit\'{e} Paris-Saclay, France}

    \affiliation{Department of Physics \& Astronomy, Northwestern University, Evanston, IL, 60208, USA}


\author{Corey Bathurst}

    \affiliation{Department of Physics, University of Florida, Gainesville, FL, 32611, USA}

\date{\today}% It is always \today, today,
             %  but any date may be explicitly specified

\begin{abstract}
%
Microcalorimeters leveraging microwave kinetic inductance detectors to read out phonon signals in the particle-absorbing target, referred to as kinetic inductance phonon-mediated (KIPM) detectors, offer an attractive detector architecture to probe dark matter (DM) down to the fermionic thermal relic mass limit. % of a few keV due to their sensitivity to sub-eV athermal phonons and native frequency-domain multiplexability. %
%
A prototype KIPM detector featuring a single aluminum resonator patterned onto a 1-gram silicon substrate was operated in the NEXUS low-background facility at Fermilab for characterization and evaluation of this detector architecture's efficacy for a dark matter search. %
%
An energy calibration was performed by exposing the bare substrate to a pulsed source of 470 nm photons, resulting in a baseline resolution on the energy absorbed by the superconductor of $2.1\pm0.2$ eV, a factor of two better than the current state-of-the-art, enabled by millisecond-scale quasiparticle lifetimes. %
%
However, due to the sub-percent phonon collection efficiency, the resolution on energy deposited in the substrate is limited to $\sigma_E=318 \pm 28$ eV. %
%
We further model the signal pulse shape as a function of device temperature to extract quasiparticle lifetimes, as well as the observed noise spectra, both of which impact the baseline resolution of the sensor. %
%

\begin{description}
\item[Report Number]
FERMILAB-PUB-23-674-LDRD-PPD
\end{description}

\end{abstract}

\keywords{Calorimeters, dark matter, kinetic inductance detectors, phonons, superconductors}
\maketitle

